(Private)-Retroactive Carbon Pricing [(P)ReCaP]: A Market-based Approach for Climate Finance and Risk Assessment

Insufficient Social Cost of Carbon (SCC) estimation methods and short-term decision-making horizons have hindered the ability of carbon emitters to properly correct for the negative externalities of climate change, as well as the capacity of nations to balance economic and climate policy. To overcome these limitations, we introduce Retrospective Social Cost of Carbon Updating (ReSCCU), a novel mechanism that corrects for these limitations as empirically measured evidence is collected. To implement ReSCCU in the context of carbon taxation, we propose Retroactive Carbon Pricing (ReCaP), a market mechanism in which polluters offload the payment of ReSCCU adjustments to insurers. To alleviate systematic risks and minimize government involvement, we introduce the Private ReCaP (PReCaP) prediction market, which could see real-world implementation based on the engagement of a few high net-worth individuals or independent institutions.

==> old/3.1_Modeling_insurance_against_Retroactive_Carbon_Pricing.tex <==
\subsubsection{Reserves for Pollution (the baseline method)}
% Tianyu is responsible for this section. Let he know if you think there are something wrong
\textit{Reserves for Pollution} works in a similar way as how \textit{Reserves for Banks} works.
Suppose $S$ is the sector space. $S = {s_1, s_2, ... s_n}$ where $n$ is the number of the sector. $Fine(s_i, sc, t)$ describe the average of historical emission fine of companies with a scale level $sc$ in $s_i$ at time t. Denote the real GDP contributed from sector $s_i$ as $GDP(s_i, t)$ at time $t$. Denoted the reserve rate as $r_t$ at time $t$.
According to the types of the companies, the government can estimate the expected carbon emission of this company by $GDP_{s_i, t}$, $Emission(s_i, sc, t)$. To avoid the case of \textit{default pollution}, which means defaulting the fine after pollution at the end of each accounting season (one year should be a reasonable guess). Thus, the \textit{Reserves funds for Pollution} of company $x$ in sector $s_i$ can be defined as $$r_t \cdot \frac{1}{m} \sum_{j = 1}^{m} GDP{s_i, t} \frac{Fine(s_i, sc(x), t-j)}{GDP(s_i, t-j)}$$
It is evident that the estimation of the fine to a certain company is the average of the GDP-readjusted fine paid by similar companies with the same scale level in the past $m$ years. The $m$ is expected not to surplus the business cycle of the section $s_i$.

When a company is registered on the market and starting to emit \textit{CO2}, a \textit{Reserves for Pollution} which is a proportion of the estimated fine will be levied. At the end of the each accounting season, if there is no default events happen, the estimated fine for the year to come should be re-evaluated and readjusted by in an retreat-more-fill-less way. However, if the company end up with not be able to pay the fine of emission at the end of a certain accounting season, the \textit{Reserves for Pollution} will not be used to pay for the fine and, as a punishment, some business activity, such as opening new factories, should be limited until the company is able to pay for the rest of the fine because the \textit{Reserves for Pollution} is not expected to be able to cover all of the fine.

\begin{itemize}
    \item pro: It is able to reduce the systematic risk of default in the market. The larger $r_t$ is, the easier to stop the default chain reaction when a minority of companies starting to default.
    \item con: Clearly, this policy is hard to be put into practice and easy to be attacked by lobbyists because it hurts the producer's passion to start a business and itself can be regarded as a significant shock to the whole economy. Thus, a reasonable $r_t$ should be carefully proposed. A large $r_t$ is safer for the whole emission trading market and, in contrast, a small $r_t$ won't have too much impact on the economics. Lastly, it's worth noticing that the concept of retreat-more-fill-less shall be shared widely in in many other methods and improvements.
\end{itemize}

\subsubsection{Vincent's PetroDollar (VPDollar)}
% Tianyu is responsible for this section. Let he know if you think there are something wrong
% source: https://www.facebook.com/yoshua.bengio/posts/3730078310430415
Instead of levying the regular tax for pollution and emission. Introducing auction is another way out to lower the risk of default. 

\paragraph{The issue process of the VPDollar}
When the customers pays for carbon intensive products, the sellers, instead of directly receiving dollars from the customers, they receive an alternative asset which we called it VPDollar from the government or a 3rd party authority financial institution like the Fed in the US (for simplicity, we use the word "government" to refer to this authority institution). The money that the sellers paid flows to the government. The value of VPDollar per unit is expected to be the equivalent in unit dollars minus some mitigation cost of the emission.

\paragraph{The Repo of VPDollar from government}
The government should hold auctions from time to time to collect the VPDollars they have issued. There can be some further discussions of the rules of the auction. A simple rule would be that before the auction the government decided an upper bound price $p_u$ of the VPDollar per unit which is remains unknown to those who participate in the auction process. VPDollar holder $i$ shall claim its own bidding $b_i$. If $b_i < p_u$, the deal is made. Otherwise, the VPDollar holder should wait until the next auction or sell the VPDollars to others in the open market.

\paragraph{The incentive of VPDollar trading between investors}
One may noticed that we mentioned the open market for VPDollar in the last paragraph. It should exist because the VPDollar's intrinsic value is given by the recollect process (the auction). Those who hold VPDollars can always get real dollars from the auctions. Thus, it's ideal that the market price of the VPDollar $p_m$ should be a rational guess of the present value of the upper bound price given by the government in the next auction. From the opposite direction, when the government define the upper bound price of $p_u$ each auction, they also should implicitly take the market price of VPDollar into consideration. If there are always too much deviation from the $p_m$ and $p_u$, investors might lose incentive to join the market. For example, every year the Federal Reserve publishes the expected inflation rate, and this expectation truly affects investors' decisions in the year to come which is exactly one of the reason they publish the expectation. Thus, they can use it as a tool to regulate macroeconomics on a small scale. However, the published rate cannot deviate too much from the real rate. Otherwise, when the Federal Reserve publishes the expected inflation rate next time, investors won't make decisions based on it.

% Vincent's original saying
%Consider a place where taxes are already charged -- say, at the pump. Instead of a regular tax, now do the following. As the customer pays a dollar for gasoline, that dollar goes to the government, and the seller in return gets a "special dollar" -- let's call it a petrodollar -- from the government. Petrodollars are not legal tender, but can be exchanged for regular dollars in the markets at whatever price they're valued at.
%Now why would anyone want petrodollars then? Intuitively, the goal is to get the value of a petrodollar to be a dollar, minus the "correct" tax. Here's one way to do that: the government commits to events (say, one every month) in which it buys back petrodollars for regular dollars. A natural way is through a reverse auction. That is, the government decides sometime in advance how many petrodollars it will buy back in the event -- ideally based on what it considers a reasonable level of polluting activity. Then those who want to sell back petrodollars place bids. A bid might be, "I will sell back up to 100k petrodollars at 0.8 regular dollars a piece." The government then accepts all bids below a certain price p (of dollars/petrodollar), pays those bidders p dollars per petrodollar, with p chosen so that the government buys back the number of petrodollars it set out to. You don't have to participate in these auctions -- you can hold your petrodollars, or you can trade them in the markets -- but this gives a basis for the petrodollars' value. If it is perceived that polluting won't seem so reasonable in the future anymore and therefore the government will buy back fewer then, then everyone will try to sell their petrodollars sooner while they still can, driving down their value and thereby in effect increasing the tax on pollution (since you always only get one petrodollar per dollar from a gasoline-buying customer).

\paragraph{Future Modification and discussion}

%\subsubsection{American Option}
% this is not really needed, financial intermediaries can create whatever derivative on the credit as required by clients


==> old/cf_cra_intro.tex <==
 
The global efforts in fighting climate change have boiled down to two broad categories of actions: (a) Climate Financing (CF), and (b) Climate Risk Assessment (CRA). 
Enormous investments are needed for mitigation efforts that can reduce emissions as well as adaption efforts that help communities adapt, thereby reducing the impacts of climate change.
CF involves funding for local, national, or transnational projects aimed at mitigating and adaptation actions for climate change. 
Not only does CF incorporate investing in green infrastructure but it also stands for financing away from activities that are harmful to the environment, e.g., deforestation, coal mining, etc. 

On the other hand, CRA is concerned with estimating the likelihood of future climate hazards and their impact on local and national communities. 
CRA helps put the long-term impacts of carbon emissions in perspective. 
For example, the effect of carbon emitted by polluters today can bring about harmful effects in future such as rising water levels and associated displacements of coastal residents. 
In mathematical terms, if we let $D$ (in monetary units) be the total economic damage due to a tonne of carbon emission today, CRA's objective is to determine the probability function $P(D)$.
Social cost of carbon is defined as the sum total of avoided future damages due to the reduction in 1 tonne of emission today. Thus, 
\begin{equation}
    SCC = E[D] = \sum_{d=0}^{\infty} d \cdot P(D=d)
\end{equation}

Various policies and projects are evaluated based on the cost-benefit analysis. 
SCC serve as a major input to determine the benefits of these activities. 
Thus, an accurate estimation of SCC is crucial for prioritization of our efforts. 
Underestimated SCC undermines polluters' impact, thereby hurting the climate financing of mitigation and adapation efforts.

For example, the governments have traditionally subsidized the activities such as coal mining for economic growth.
However, this has come at the cost of GHG emissions harmful to the environment. 
In addition to subsidies to support growth, governments have also underpriced energy compared with social costs (such as damage to health and the environment). 
This has been termed as implicit subsidy by researchers~\cite{parry2021still}.

Due to the the longer time scales at which the harmful effects of emissions show up, the probabilisitic structure of economic damages $P(D)$ is hard to determine~\cite{nordhaus2017evolution}. 
This uncertainty is exacerbated by ``tragedy of horizons", wherein agents such as corporations, governments, and households have different horizons to consider for decision making~\cite{carney2015breaking}. 
Integrated Assessment Models (IAMs) have been used to determine various ways in which future can unroll. 
In a systematic study ~\cite{nordhaus2017integrated} concludes that IAMs vary in their complexity, with each type having its own advantages and disadvantages. 
We lack the sophistication of physical and socioeconomic analysis to accurately predict what will be the climate disasters in the future or which political views will drive the future economies. 

However imprecise CRA is at the moment, it is still an important input to prioritize adaptation and mitigation actions, i.e., climate financing.
A poor risk assessment yields poor climate financing, thereby slowing our progress towards addressing climate change. 
Similarly, a more accurate risk assessment will help governments, investors, and communities to funnel appropriate funding to climate financing activities. 

The urgency of transition to a net-zero economy can’t be stressed enough. 
This has been on the agenda of the COP since the ringing of the first warning in 1995. 
Each year COPs result in treaties and ever more ambitious NDCs but without any enforcement and accountability bodies. 
As a result, these pledges are good as far as they can go.
Among several reasons for more aggressive action, one reason being commonly addressed through TSVCM is the standardization of carbon accounting. 
In line with this reasoning, we propose an independent mechanism that has the potential to serve as a global reference or standard for continually improving CRA, thereby leading to appropriate CF. 

Our proposal, discussed in Section~\ref{sec:rcp}, serves the following purposes 
\begin{itemize}
    \item Encourages model innovation to estimate SCC, thereby improving CRA
    \item Funnels an appropriate amount of funds to climate change mitigation and adaptation efforts, thereby improving CF
\end{itemize}

==> old/cfa-cra.tex <==
\subsection{Climate Finance: Executing the balancing act}

Carbon pricing must execute a balancing act in order to optimize its fundamental role in policy and investment decision-making across governments, institutions, and companies. 
Governments use a carbon price in attempts to optimize the balance between economic productivity and GHG reduction. 
Companies use internal carbon prices in their cost-benefits analyses regarding corporate strategies and capital allocations to assess the burden of emissions (i.e., anticipated future damages) on their balance sheets. 
The appeal of a carbon price lies in its ability to maximize flexibility for economic actors whilst appropriately minimizing emissions. 
While carbon pricing may take many forms, a coordinated price can effectively mobilize capital towards low-carbon innovations and business models. 
Therefore, carbon pricing, and executing the balancing act, would influence the financial system to catalyze a net-zero transition in the form of climate finance.

\subsection{Climate Risk Assessment}

Better SCC estimates matter. 
Currently, the price of GHG emissions influences many facets of regulatory and business behavior. As climate change concerns take the global center stage, the SCC’s influence may span new avenues, including, but not limited to, legal and social risk management. 
Therefore, the value’s growing significance urges the need for more robust SCC estimates to encourage optimal economic, environmental, and social behavior.

In the public sector, the SCC benchmark influences policy design and evaluation by enhancing cost-benefits analyses.
Quantifying the monetary benefits of emissions regulation improves government agencies’ ability in implementing sound, viable regulations.
The UK government, for instance, continues to centers much of its energy- and emissions-related regulatory activities on the SCC \citep{Watkiss}.
Moreover, the SCC enables public electric utilities to capture a more complete cost-benefits analysis of various actions thereby improving resource planning \citep{CaliforniaEnergyCommission2021}. 
The use of SCC in government policy, however, is not met without criticism \citep{Auffhammer2020}, \citep{Stern2021}, questioning robustness of the value estimation. 

As the public sector uses the SCC to determine policies and regulations, the private sector assesses strategies and investments in anticipation of such shifts. 
Businesses and investors implement SCC estimations to identify potential risks and opportunities. 
The former uses internal carbon pricing to monetize the impacts of their operations on the climate as well as forecast project exposure to carbon regulations \citep{Fan2021}. 
BP, for instance, stress tests its large new projects in industrialized economies with a \$40/tCO2e value \citep{Ahluwalia2017}.
Investors, also, use SCC estimates and internal carbon pricing to analyze policy interventions’ impacts on their portfolio as well as identify the climate impacts of potential investment opportunities \citep{Fischer2020}.
Despite carbon pricing’s emerging prominence in the private sector, many companies’ and investors’ internal carbon prices remain undisclosed \citep{Bartlett2021}. 
Even if they are disclosed, current pricing thresholds are found to vary significantly, a majority of which remain lower than what is required to achieve climate goals \citep{Fan2021}.
Without improved certainty and estimation of the SCC, such climate-incompatible behavior may persist.

In this paper, we introduce a new scheme to internalize climate change negative externalities.
In contrast to the Pigouvian tax, our Retroactive Social Cost of Carbon Updating (ReSCCU) scheme levy the tax in a retrospective way so that the every dollar accounts for long-term negative impact from CO2 emission to the environment.
Because it is hard for individuals to estimate the price of future carbon, we put forward Retroactive Carbon Pricing (ReCap) scheme which allows individuals only pay for fixed cash flow each year and transfer the burden of estimating social cost of carbon (SCC) by swap contracts to large financial institutes where estimating SCC are easier because they have advantages on information flows.

In time, a good estimation of social cost of carbon will be made and authorities can make reasonable policies referring to these estimations, so that we can take action wise precautions and get alert before climate catastrophe could happen. 


==> old/intro-v2.tex <==
\section{Introduction}
Climate change potentially poses incredible risks to our environmental, economic, and social well-being. Policymakers have convened \citep{UNFCCC2015} to discuss how to limit the increase in global mean temperature, thus reduce climate change risks, to 2°C or less by decreasing greenhouse gas (GHG) emissions. To achieve ambitious climate goals, a global low-carbon energy transition, the shift away from fossil-fuel-based energy systems, is required. While many solutions exist to materialize an energy transition, the current economic, political, and social incentive structures are misaligned with what is needed to reduce emissions and promote well-being \citep{OECD2019}. For instance, the number of coal and gas-fired power plants continue rise in some countries as they look to acquire affordable, reliable energy despite the plants’ known contributions to climate change \citep{Greenfield2021a}, \citep{Greenfield2021b}. Free markets’ inability to maximize society’s welfare deems climate change as a market failure \citep{Benjamin2007}. The implications of rising GHG emissions are considered external to markets; therefore, as economic theory argues, failure to internalize social marginal damages will lead to the overproduction of negative externalities. To discourage this behavior, and shift capital towards low-carbon opportunities, economists suggest setting a price on GHG emissions.

GHG pricing, referred to as carbon pricing, is an economic instrument that captures the costs of net damages incurred from one additional ton of emissions in a given year. Carbon pricing incorporates climate risks into policy and investment decisions, thereby placing the burden of emissions on emitters. The mechanism emerges in two market-based approaches: a carbon tax and a cap-and-trade system, also known as an emissions trading scheme (ETS). The former is a Pigouvian tax \citep{Pigou1920}, a tax on a market activity that generates negative externalities; the latter allows emitters to trade a fixed supply of emissions allowances set by the policymakers and an equilibrium price is found amongst the suppliers and buyers \citep{Dales1968}. Regardless of the approach used, economists \citep{Nordhaus2017} emphasize the need to establish a carbon price that is reflective of the monetized social marginal damages from emissions known as the social cost of carbon (SCC).

The SCC represents the present value of future damages incurred by an incremental ton of carbon-equivalent emissions. This high-level number serves as the most-efficient method to inform policy and investment decision-making. An increasing number of governments and financial institutions measure the cost-benefits of their decisions by using the SCC. Finding the optimal SCC, however, proves cumbersome. Its calculation requires executing the balancing act between short-term, carbon-driven economic productivity and long-term, carbon-driven climate risks. Scientists estimate the SCC using Integrated Assessment Models (IAMs) \citep{Nordhaus2020}, \citep{Hope2011}, \citep{Tol} that capture dynamics of the economy, atmosphere, ocean and other social and physical systems. Despite their significance in current climate policy and finance, IAMs fall short in many respects, from their outdated nature and inability to account for uncertainty. As climate begins to take precedence in decision-making and technological capabilities exponentiate, the SCC is ripe for model innovation that better reflects the true cost of climate damages.

Here, we propose a novel market-driven SCC benchmark signal to unlock realistic carbon pricing by retroactively adjusting prices. We first explore carbon pricing's balancing act, it's role in climate finance, and its influence across policy and markets. Afterwards, we assess prior market and modeling-based approaches. Next, we introduce retroactive carbon pricing. Then, we contextualize market-based retroactive carbon pricing. Finally, we discuss advantages and disadvantages of our model before presenting conclusions and future work.

\subsection{Climate Finance: Executing the balancing act}

Carbon pricing must execute a balancing act in order to optimize its fundamental role in policy and investment decision-making across governments, institutions, and companies. 
Governments use a carbon price in attempts to optimize the balance between economic productivity and GHG reduction. 
Companies use internal carbon prices in their cost-benefits analyses regarding corporate strategies and capital allocations to assess the burden of emissions (i.e., anticipated future damages) on their balance sheets. 
The appeal of a carbon price lies in its ability to maximize flexibility for economic actors whilst appropriately minimizing emissions. 
While carbon pricing may take many forms, a coordinated price can effectively mobilize capital towards low-carbon innovations and business models. 
Therefore, carbon pricing, and executing the balancing act, would influence the financial system to catalyze a global energy transition in the form of climate finance.

\subsection{Climate finance and the ‘tragedy of the horizon’}

Climate finance addresses the need to reallocate significant amounts of capital needed to materialize a low-carbon transition \citep{McCollum2018}. Despite concerted efforts to limit emissions and temperature increase, deep decarbonization has yet to be realized as fossil fuel growth persists \citep{Jackson2019}. The former Governor of the Bank of England, Mark Carney, noted this trend and called for the massive reallocation of capital towards low-carbon warning to avoid damaging climate-related risks \citep{carney2015breaking}. In his speech, Carney urges the need to break the `tragedy of the horizons’–wherein business, political, and technocratic cycles are measured in a few years as opposed to the time horizon of climate change–to mitigate risks of climate change and financial instability. While carbon pricing may effectively mobilize climate finance and answer Carney’s calls, the risks associated with miscalculating a carbon price, particularly the SCC, are nontrivial.

The SCC estimations are susceptible to their own `tragedy of the horizon’ which imposes consequences on economic and social actors. For instance, economists are not in agreement on how to determine the appropriate discount rate for climate damages. One side \citep{Stern2007} argues for the prescriptive approach–assuming a discount rate (e.g., 1.4\%) conforming to ethical ideals–while the other \citep{Nordhaus2007}, \citep{Nordhaus2017} argues for the descriptive approach–a discount rate (e.g., 4.25\%) based on observable returns on real assets. The difference in applied discount rates results in conflicting estimations on what is an ‘optimal’ SCC. Such conflicts, therefore, cause confusion and imbalances in carbon pricing benchmarks. These `sub-optimal’ benchmarks will either slow an energy transition and exacerbate climate risks or erroneously allocate capital and deter economic productivity. Attempting to break the `tragedy of the horizon’ by relying on an average SCC would undermine its global influence and the future damages of climate change.

\subsection{SCC Influences}

Better SCC estimates matter. Currently, the price of GHG emissions influences many facets of regulatory and business behavior. As climate change concerns take the global center stage, the SCC’s influence may span new avenues, including, but not limited to, legal and social risk management. Therefore, the value’s growing significance urges the need for more robust SCC estimates to encourage optimal economic, environmental, and social behavior.

In the public sector, the SCC benchmark influences policy design and evaluation by enhancing cost-benefits analyses. Quantifying the monetary benefits of emissions regulation improves government agencies’ ability in implementing sound, viable regulations. The UK government, for instance, continues to centers much of its energy- and emissions-related regulatory activities on the SCC \citep{Watkiss}. Moreover, the SCC enables public electric utilities to capture a more complete cost-benefits analysis of various actions thereby improving resource planning \citep{CaliforniaEnergyCommission2021}. The use of SCC in government policy, however, is not met without criticism \citep{Auffhammer2020}, \citep{Stern2021}, questioning robustness of the value estimation. 

As the public sector uses the SCC to determine policies and regulations, the private sector assesses strategies and investments in anticipation of such shifts. Businesses and investors implement SCC estimations to identify potential risks and opportunities. The former uses internal carbon pricing to monetize the impacts of their operations on the climate as well as forecast project exposure to carbon regulations \citep{Fan2021}. BP, for instance, stress tests its large new projects in industrialized economies with a \$40/tCO2e value \citep{Ahluwalia2017}. Investors, also, use SCC estimates and internal carbon pricing to analyze policy interventions’ impacts on their portfolio as well as identify the climate impacts of potential investment opportunities \citep{Fischer2020}. Despite carbon pricing’s emerging prominence in the private sector, many companies’ and investors’ internal carbon prices remain undisclosed \citep{Bartlett2021}. Even if they are disclosed, current pricing thresholds are found to vary significantly, a majority of which remain lower than what is required to achieve climate goals \citep{Fan2021}. Without improved certainty and estimation of the SCC, such climate-incompatible behavior may persist.

% TODO: Need to add more on future, potential influences of SCC e.g., legal and political risks; emphasize why the SCC matters!!!

% TODO: related work
% Market-based approaches: Tax and ETS (necessary??)
% Model-based: IAMs
% --> Discounting
% --> Damage function (talk w/ andrew)

\subsection{Climate Risk Assessment}

% Story in a nutshell: Finance needs interest benchmarks. The energy transition requires these to be more long-term and SCC-aware. Current benchmark rates are not fit for purpose (LIBOR, SOFR, but also long-term treasury swap rates). We suggest a novel mechanism for revealing a long-term SCC benchmark signal through retroactive carbon pricing. In doing so, we follow recent trends (e.g. SOFR and €STR) in working with market-based mechanisms, however, unlike existing trends, we argue that SCC prediction requires the creation of a novel market type tat is subject to customised rules.
% NOTE: We don't know yet whether this story is any good!

In order to keep global warming to safe levels, the world needs to undergo both mitigation and adaptation actions. 
To this end, we need to be able to assess the economic damage due to carbon emissions for two reasons: First, policymakers need to be able to evaluate and compare the economic consequences of a large variety of possible policy pathways, and secondly, the principle of \textit{polluter pays} demands that emitters pay for the economic damages inflicted by their emissions.

A unit of carbon emitted into the atmosphere will remain there for a very long time, during which it will continuously contribute to the overall economic damages caused by global warming. 
The \textit{social cost of carbon (SCC)} denotes the cumulative lifetime economic damage caused by releasing an additional unit of carbon into the atmosphere.
Calculating the SCC in advance requires both physical and socioeconomic modeling of the future, making SCC estimates subject to numerous sources of uncertainty. 
Consequently, SCC estimates of past emissions become more accurate as hindsight increases. 

Society benefits from improved SCC forecasts in numerous ways: They enable policymakers to make more informed counterfactual decision-making, and give activists and politicians a stronger case for preventative action. 
Improving SCC forecasts, however, also carries an explicit marginal economic value arising from a variety of demand sources: Governments may wish to charge polluters appropriately, and in a timely manner to reduce defaulting risk. 
Insurance companies may wish to establish appropriate premiums for insuring polluters from future compensation. 
Investors and creditors need to know a company's exposure to future compensation payments. 

Today, banks and other financial institutions use so-called benchmark references such as LIBOR (and soon, SOFR) for determining interest rates for debt instruments, as well as mortgage conditions, corporate loans, government bonds, credit cards and even student loans. 
These existing benchmarks alone, however, were not designed to, and are arguably not fit-for-purpose to guide the global financial industry's transition to a net-zero world.

First of all, financing the global economy's decarbonisation requires investment commitments at both unprecedented volumes and, possibly decadal, horizons. 
LIBOR or SOFR future rates, however, are fixed for maturities for up to 12 months. Derivatives markets, such as derivatives on EURIBOR rates, have forwards up to $50$ years in advance, and benchmarks such as ICE have swap rates available for G5 currencies up to $30$ years in advance.  
The underlying markets have not been designed with the unprecedented risk of climate change and the energy transition in mind: These markets are for general-purpose interest rate trades, i.e. long term predictions of central bank interest rate policies and inter-bank secured lending.  Because most activities in finance now have horizons of only a couple of years, these markets are much less liquid beyond the 10 year point, and quite illiquid at $30$ and $50$ years. This simply is so because so few economic agents plan/trade with forecasts for that horizon, and as such the predictions generated in this market are not complete (i.e., not beyond the $30$ year point), or unreliable due to low liquidity. 
Nevertheless, banks and other financial institutions do frequently base their long-term interest rates on short-term benchmarks, thus exposing them to basis risk. We argue that the challenges of the energy transition require the creation of novel, long-term interest benchmark signals that help market participants manage risks associated with SCC uncertainty in a standardized way. 
% managing the risks associated with SCC forecasting volatility

A SCC benchmark based on surveys among climate insurers would be exposed to much the same vulnerabilities that led to LIBOR's discontinuation, including intransparency and susceptibility to manipulation. 
Fundamental analysis of insurance company balance sheets is limited to public information. 
Forcing insurance companies to reveal private information to independent benchmark agencies, such as governments, seem both politically infeasible and intransparent.

SOFR, LIBOR's successor benchmark, is instead derived from trading data on the US Treasury's repurchase agreement (repo) market. 
Daily transaction volumes frequently exceeding USD $1$ trillion are deemed to strengthen SOFR's reliability. 
Other short-term benchmark rates, such as €STR, have followed similar, market-based approaches. 
In this paper, we explore the feasibility of establishing a long-term SCC benchmark rate. 


==> old/limitation_carbon_tax.tex <==

\label{sec:resccu-tax}

% In the previous section, we have introduced ReSCCU, which we suggest should replace the social cost of carbon (SCC) as a metric for policy decision making. 
% Although we give a formal definition of ReSCCU's continual readjustment mechanism, we do not detail how to implement it in practice.

A \textit{carbon tax} is a mechanism through which a government charges polluters, usually companies, according to their GHG emissions. 
Carbon taxes aim to align \textit{private firms} with \textit{social good}.
First, charging a carbon tax pools funds that the government can use in order to pay for communal damages created due to pollution events.
It is established practice in international environmental law that a polluter should pay for the totality of the damages it is responsible for, as encoded in the \textit{polluter pays principle (PPP)} \citep{tokuc_rio_2013}. 

Second, the act of charging polluters may by itself deter polluters from \textit{overproduction} of goods, thus restoring market equilibria distorted by a lack of internalization of externalities.
Both of these aspects are captured by the concept of \textit{Pigouvian tax}~\citep{Pigou1920}, which internalises externalities, such as pollution, by modifying the maximum of the consumer utility function. 
~\citet{Pigou1920} showed that the consumer's choice coincides with the socially optimal investment level iff Pigouvian tax is set to the marginal pollution damage. 

As we establish in the following section ( Section~\ref{sec:resccu}), calculating the damage inflicted due to an additional ton of CO2 (or CO2-equivalent) released into the atmosphere is inherently difficult.
If a ton of CO2 is released into the atmosphere today, half of it will still remain there after $30$ years, and a fifth of it even after hundreds of years. 
Even if a polluter applies artificial technological means to remove an extra ton of CO2 from the atmosphere at a later date, it is possible that damage continues to occur due to system hysteresis. 
GHG pollution events are therefore inherently \textit{temporally extended over a long time horizon}. 
Pigouvian taxation was proposed long before anthropogenic climate change became a wide economic cause for concern. 
Consequently,~\citet{Pigou1920} did not consider the case that Pigovian tax could be hard, or indeed impossible, to calculate and, furthermore, only be estimated under not-so-significant uncertainty. 

The question of whether, and if so, how, to price in uncertainties in estimating the SCC to fix prices for Pigouvian tax has been raised soon after its adoption in 2009.
Indeed,~\citep{metcalf_design_2009} suggested that an optimally designed carbon tax would respond to uncertainty by continuously updating the tax rate ``as new information becomes available about the costs and benefits of reducing emissions''. 
In the face of uncertainty about the costs of abatement, the best available option was to ``utilize a crude estimate of the optimal rate and adjust the rate as new information arises''.
However,~\citet{metcalf_design_2009} does not distinguish between irreducible (aleatoric) prediction errors, and epistemic errors, the latter being in principle avoidable in the limit of sufficient data collection and model calibration.

Further,~\citet{kousky_risk_2011} argue that SCC estimates should carry a \textit{risk premium}, reflecting that each abated ton of GHG emissions would also thin the fat-tail of low-probability, high-impact, catastrophic damage events.
Risk-aversion, in such a situation, would command paying a, potentially significant, positive surcharge on the SCC in order to not only reduce the mean, but also the variance of losses through emissions abatement. 
Such an argument is in line with the so-called \textit{precautionary principle}, defined by \citet{sunstein_irreversible_2006} as \blockquote{\textit{when regulators are dealing with an irreversible loss, and when they
are uncertain about the timing and likelihood of that loss, they should
be willing to pay a sum – the option value – in order to maintain
flexibility for the future.}}
However, \citet{kousky_risk_2011} do not provide a preferred mechanism by which a risk premium should be calculated.

Finally,~\citet{weisbach_should_2012} counters that the precautionary principle was not applicable to Pigouvian taxes and that government shall charge simply the ``expected marginal social harm from an activity, adjusted in each period to reflect new information.''
\citet{weisbach_should_2012} justifies this conclusion by arguing that 
\blockquote{\textit{[...] environmental taxes decentralize decision-making. They impose a price on harm-causing activities and let individual actors decide the appropriate level of activity given that price. Individual actors will take precautions if appropriate. We can think of Pigouvian taxes as completing the market, and like in other situations with complete markets, we rely on individuals to determine the appropriate level and timing of their activities. The government should not additionally accelerate or delay environmental taxes.}}

This conclusion relies on a number of limitations.
First, any estimation of marginal harms would need to be based on knowledge about to what extent individual actors take precautions.
However, it is entirely unclear to what extent precautionary attitudes can be predicted in advance: even in the absence of climate change effects, precautionary attitudes can change rapidly in response to unprecedented events, as evidenced by the COVID-19 pandemic \citep{thoma_cognitive_2021}. 
Second, taxes are required to ``adjust to new information'' such that estimates of damages from earlier emissions can be revised, and thereby adjusting the future behavior.
However, given the global nature of the negative externalities associated to carbon emissions, it is not clear if this information is readily available in a setting with multiple actors making decisions related to emissions.
In other words, if assessing the impact of previous actions on total emissions and damages is difficult, then it is also nontrivial to adjust future emissions without some form of global cooperation or information sharing. 
Third, \citet{weisbach_should_2012} notes that their analysis relies on the price on pollution not to affect the pace of technological development.
Finally, the authors do not account for a large proportion of unskilled market participants like small and medium-sized enterprises (SMEs) that are subject to the \textit{Tragedy of the Horizon} and lack resources (e.g., qualified staff) to assess climate risks.

As SCC models cannot be guaranteed to be free from \textit{epistemic errors} even in the absence of \textit{environment (aleatoric) uncertainty}, \textbf{we propose} that, in the context of Pigouvian taxation, \textbf{the precautionary principle does indeed need to be applied to SCC estimates}.
Unlike well-known prior criticism of established SCC models, including DICE and RICE \citep{Stern2021}, we base our proposal primarily on the observation that the current \textit{model innovation process} for integrated assessment models (IAMs) is not optimal. 
This is immediately the case due to the lack of a reliable and transparent mechanism to assess \textit{retrospective global climate damages} that prohibits the \textit{calibration} of any SCC models to real-world data, as well as the lack of an incentive to develop such a mechanism. 
However, even if such a mechanism became available, we argue that the innovation process of SCC models should not rely solely on academic innovation by a small group of intellectuals, but rather on decentralized decision-making by skilled market participants - a central tenet in neoclassical economic theory \citep{weisbach_should_2012}. 

Assuming the existence of a commonly agreed methodology for measuring retrospective marginal damages, at first glance, a fair way of charging polluters would therefore be through establishing a long-term liability where polluters are periodically charged with the marginal damages incurred so far. 
According to neoclassical economics, this liability should, in general, incentivise decentralised decision makers to take future climate risks into account \citep{weisbach_should_2012}. 
In contrast, Pigouvian tax is generally interpreted as a one-time charge at the time of pollution. 
We note that there are two important practical reasons for why polluters should be charged in advance.
Firstly, due to the short decision-making horizons of polluters it is not guaranteed that they will price in their long-term liabilities adequately, thereby hampering the mitigation of long-term climate risks.
Second, compensation from polluters often needs to be pooled-in to finance long-term investments into adaptation and mitigation measures.

Thus, in the subsequent sections, we introduce our proposed mechanisms to address the aforementioned disadvantages of one-time fixed carbon taxes and difficulty of estimating SCC.

==> old/old-paper-retroexchange.tex <==

In this section, we describe a hypothetical market that deals in ReCaP, addressing the various issues such as fostering model innovation described in the previous sections. 
We further discuss various incentives for the sellers, buyers, and mediators involved therein. 

\subsection{RetroExchange}

\begin{figure}
    \centering
    \includegraphics{images/exchange.png}
    \caption{Diagram from slides go here}
    \label{fig:exchange}
\end{figure}

Sellers list uninsured (UICCs) or insured (ICC) carbon credits with the RetroExchange at whatever asking price and volume they want.
Any carbon credit that has not yet been converted to an insured carbon credits (ICC) by the RetroExchange is assumed to be uninsured (UICC).
Buyers bid on the RetroExchange for insured carbon credits (ICCs) - uninsured credits are not purchasable. 
Insurance companies offer insurance contracts for credits. 
The bundle of a carbon credit and an insurance form an ICC. 
Insurers operate on the sell side of the exchange and post the asked insurance premium, and they post the volumes of insurance contracts they are willing to sell. 
For simplicity, let's assume all retroactive payments are capped to $30$ years since conversion from UICC to ICC \footnote{Otherwise we need to distinguish between ICCs of different maturities}.

The clearing mechanism by the RetroExchange is now a sealed-bid auction with a complication: 
While ICCs can be cleared straightforwardly, UICCs need to be cleared according to a novel 3-agent auction - i.e. the RetroExchange clearing mechanism needs to convert UICCs into ICCs according to whether the combined price of supplier ask and insurer premium asks can satisfy buyer bids. 
The insurer premium can be regarded as a variable added transaction cost.

Who will buy ICCs? What are the scenarios?

Suppose we know the number of insurance contracts the insurers $j = 1\ldots J$ are willing to underwrite through the insurer specific supply function $S^j(p(t), \mathbb{E}_t [ SCC ])$, where $p$ is the premium.
Suppose also we know for each polluter $i=1,\ldots I$ the demand for credits as a function of the premium amount and the initial SCC charge 

Generally, the premium $p(t)$ is market-clearing when

\begin{equation}\label{equation:clearing}
\sum_j^{J} S^j(p(t), \mathbb{E}_t [ SCC ]) = \sum_i^{I} D^i(p(t), \mathbb{E}_t [ SCC ]) \text{ holds}.
\end{equation}

Different market mechanisms try to find one or more market clearing premiums $p(t)$ in different ways, and many proposed mechanisms to find clearing prices are intractable unless the shape of demand and supply functions are constrained. 
Without restricting the shape of demand and supply functions, organising an auction can be costly in terms of computation and communication between agents and the auction organisers. 
Therefore in the real world markets often operate mechanisms that are constantly in disequilibrium (such as the double auction), but which approximate the equilibrium prices nonetheless.
Therefore the choice of market mechanism, and the rationality with which the agents execute their orders in a disequilibrium market mechanism determine how successful the market is in satisfying agents preferences.

In economic models however, frequently convenient restrictions are placed on the supply- and demand-functions. Oftentimes, demand is assumed to be decreasing in price. 

Insurer competition is induced by the RetroExchange trying to minimise the combined asking price, i.e. insurer asks with lower premiums are preferred. Winning insurance premium bids result in swap contracts (or new instruments NI) between the winning insurer and the RetroExchange. 

\subsection{Risk Management}
Risk management: The RetroExchange bears the insurance default risk. 
When an insurer goes bankrupt, this means that any associated outstanding retroactive payments will not be covered, but also that any outstanding claims will not enacted.
Hence, insurance default may not necessarily be unprofitable to the RetroExchange.
The RetroExchange takes furthermore the risks associated with being on the other side of the swap contracts. 
This means that large negative retroactive adjustments might cause the RetroExchange to go bankrupt, in which case the the insurances would bear the RetroExchange default risk. 
Systematic risks can be lowered by traditional ways (i.e. require insurers to have reserves, reinsurance etc, proper premium pricing). systematic risk, namely the failure of the RetroExchange and clients due to a cascading default of one client (polluter or insurer) is prevented through buffers (initial margin, variation margin) held at the exchange in correspondence with the market reforms that were enacted after the Global Financial Crisis (Dodd Frank in the US, EMIR in the EU). 
The RetroExchange is expected to receive a revenue stream from selling the SCC signal derived from the insurance premium spreads observed (these are only revealed to the RetroExchange, and are not publicly available). 
A special way of lowering system risk is to require the RetroAgency's cumulative pricing adjustments to be bounded - this interferes with the quality of the SCC signal, but may be a sensible way to deal with extreme value risks on the tail.

\subsection{Towards ``true" SCC}
Derivation of the SCC signal. The RetroExchange observes the insurance premium spread at each transaction (independently of whether UICC to ICC conversion takes place or not). The insurance premium spread itself is, however, confounded by a) speculators or bets on the future SCC, b) finite horizon of the NI, as well as c) price adjustments aiming to hedge against future business risks, or recovering from past mistakes. 
Past mistakes can be detected by the RetroExchange (and hence potentially adjusted for), and insurance hedging behaviour should be minimized by the competition between insurers.

In this way, it is ensured that a) each carbon credit traded on the RetroExchange is insured once and b) both buyers and sellers are completely unexposed to the retroactive carbon pricing mechanisms - to them, the RetroExchange feels like an ordinary exchange. Carbon credits can be traded across other exchanges as long as any UICC is first converted to an ICC before traded on the RetroExchange (ICCs can be sold at any other exchange if needed - to other exchanges, they are just ordinary carbon credits).

\subsection{Voluntary participation}
% We argue that getting governments on board is hard, and not a good first step toward deployment. We argue that a market approach that creates an artificial insurance market is best for early deployment, and this should be incorporated into voluntary carbon markets (TSVCM).
% RetroAgency, RetroExchange etc are introduced here


Reasons to participate in centralized markets:

\begin{itemize}
    \item Banks may have clients that need emissions allowances. A centralized market offers more liquidity, and is therefore expected to offer better prices than a decentralized market.
    
    \item  Diversification of other risks, in the literature on catastrophe risk it is shown that catastrophe risk insurance as an investment has small correlation to other market indices. Though it is unclear if this would hold for climate risks due to pollution as well, since there is a causal link between economic activity and carbon outputs.
\end{itemize}



==> old/private_recap.tex <==
\label{sec:precap}

In Section~\ref{sec:recap}, we introduced ReCaP as an application of ReSCCU to Pigouvian taxation. 
While, in theory, ReCaP improves over SCC-based taxation, it also poses a few practical challenges grounded in risk diversification as well as large-scale political buy-in and systemic relevance. 
In face of these obstacles, and as a complementary measure, it does serve well to consider: What can private investors do in order to help implement ReSCCU?

In this section, we introduce \textit{Private ReCaP (PReCaP)}, a novel mechanism that enables ReSCCU to be implemented without requiring the government buy-in while preserving the benefits of ReCaP and offering additional advantages in terms of climate financing.
Importantly, unlike ReCaP, PReCaP could, in principle, see real-world implementation based on the engagement of a few high net-worth individuals or independent institutions as well as a minimal participation from the government. 

\subsection{The PReCAP prediction market}

In its basic form, PReCaP implements competitive incentives between a group of insurance companies within the context of a \textit{prediction market} (also called \textit{betting market})\footnote{Note that these aren't strictly insurances as they do not actually "insure" any real-world assets in the conventional sense.} that are trying to predict future ReSCCU adjustments estimated by a trusted RetroAgency. 
This is achieved by creating a market for insurance policies in which demand is stimulated artificially by a sponsoring agency, which we dub the RetroExchange, which can, in turn, derive a decentralized market estimate of $SCC_t-\widehat{SCC}_t$ based on the spread of insurance premiums offered by the insurance companies (see Figure \ref{fig:precap}). 

\paragraph{Risk management.} The RetroExchange bears the insurance default risk. 
When an insurer goes bankrupt, this means that any associated outstanding retroactive payments will not be covered, but also that any outstanding claims will not be enacted.
Hence, insurance default may not necessarily be unprofitable to the RetroExchange.
The RetroExchange takes furthermore the risks associated with being on the other side of the swap contracts. 
This means that large negative retroactive adjustments might cause the RetroExchange to go bankrupt, in which case the the insurances would bear the RetroExchange default risk. 
Such systematic risks can be lowered by traditional ways, e.g.,  requiring insurers to have reserves posted with the exchange in a default fund, or through reinsurance.  
% Other risks due to a cascading default of one client (polluter or insurer) is prevented through buffers (initial margin, variation margin) held at the exchange in correspondence with the market reforms that were enacted after the Global Financial Crisis (Dodd Frank in the US, EMIR in the EU). 
Other ways to safeguard against such defaults can include flooring RetroAgency's cumulative pricing adjustments, which may interfere with the quality of the SCC signal, but may be a sensible way to deal with extreme value risks on the tail.
Further, RetroExchange might benefit from the revenue stream by selling the SCC signal derived from the observed insurance premium spreads as these will only be revealed to the RetroExchange (see Appendix C for derivation of the SCC signal). 
% An special way of lowering system risk is to require the RetroAgency's cumulative pricing adjustments to be bounded - this interferes with the quality of the SCC signal, but may be a sensible way to deal with extreme value risks on the tail.

% We argue that getting governments on board is hard, and not a good first step toward deployment. We argue that a market approach that creates an artificial insurance market is best for early deployment, and this should be incorporated into voluntary carbon markets (TSVCM).
% RetroAgency, RetroExchange etc are introduced here


\subsection{PReCaP as a breakthrough technology investment}

While PReCaP does not implement the polluter-pays principle for greenhouse gas emissions in full, we here discuss a way in which polluters could be charged with the costs of model innovation for SCC estimation, thus internalizing part of the mitigation costs. 
This may be achieved by implementing PReCaP in the context of voluntary carbon markets, as spearheaded by the Taskforce on Scaling Voluntary Carbon Markets (TSVCM). 

TSVCM has long recognized the centrality of the challenge to divert sufficient cash flows to breakthrough technologies, i.e. early-stage technologies that currently create carbon credits at uncompetitive prices (we dub these \textit{breakthrough credits}). 
In fact, \citet[Final Report]{tsvcm_taskforce_2021} observes that:

\begin{quote}
Many of the investments needed to scale
emerging breakthrough technologies do
not meet the risk and return expectations of
today’s markets. A range of mechanisms will
be needed to ensure capital flows to these
technologies. These could include blended
financing, access to benefit markets (including
voluntary carbon markets), or altering risk,
return or time horizon expectations for
projects with the highest potential for climate
impact. [...] For finance to flow to these GHG emissions
avoidance/reduction and removal/
sequestration projects, well-functioning
voluntary carbon markets will be a critical
enabler.
\end{quote}

As an alternative approach to these challenges, we propose to introduce regulation that would require polluters to acquire a fixed percentage of their carbon offsetting credits from breakthrough credit suppliers. 
To prevent market manipulation, the price of such breakthrough credits would be capped at the social cost of carbon (SCC).

In theory, such a mechanism would enable a sizable amount of cash to be diverted from polluters to breakthrough technology innovators: Even a modest $10\%$ requirement and a modest SCC of USD$100$ per ton could, according to TSVCM predictions, result in tens of billions (and up to hundreds of billions) of USD being diverted to breakthrough technologies by 2030\footnote{Assuming a demand of 1-2 Gt CO$2$ by 2030 \cite{tsvcm_taskforce_2021}.}. 
Politically, such regulation may find substantial backing due to its ability to both efficiently tackle the breakthrough technology innovation problem, while implementing a pure form of the polluter pays principle.

The challenge with this approach is, of course, that it requires fixing a suitable SCC level as SCC estimates defined through political processes tend to be both too low from a climate safety, as well as from a volume of total breakthrough subsidies aspect. One option would be to fix the SCC in line with what the IPCC deems safe \cite{ipcc_global_2018}. 

However, this setup itself does not address the need for SCC model innovation, which we argue to be just another form of a breakthrough technology. The simplest way to incorporate SCC model innovation into our setup would be to levy a small surcharge on top of the current SCC estimate which would then be diverted to e.g. academic grants to SCC research. However, in this paper, we have outlined that such a reinvestment may not be particularly efficient.

In the next section, we describe how, instead, ReSCCU could replace the SCC in such a setting, resulting in SCC estimates that would correct themselves over time, and subsidizing SCC model development through the creation of a SCC prediction market.

\subsection{Insuring carbon credits: A mechanism to charge for model innovation}

Having discussed the financing of breakthrough technology innovation as a core challenge to TSVCM, we now propose a detailed mechanism for how ReSCCU surcharges could be implemented in the context of a voluntary carbon market based on a form of a scalable \textit{symbolic insurance} for carbon credits. 

Central to this ambition is the realization that stock exchanges trading carbon credits, due to their pre-existing infrastructure and in-house skills, may rather naturally assume the role of a suitable sponsoring agency for PReCaP.
Additionally, polluters acquiring carbon credits from suppliers can easily be charged with ReSCCU model innovation costs if such a \textit{RetroExchange} requires each carbon credit to be \textit{insured}.
Together, this gives rise to a decentralised market mechanism that both stimulates model innovation as well as reveals an improved SCC estimate while being financially sustained by polluters - a proposal very much in the spirit of the polluter-pays principle.

\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\linewidth]{images/MarketReCaP_v2.png}
    \caption{Private ReCaP. (a) An independent RetroAgency devises a SCC machine. (b) A RetroExchange chooses a RetroAgency’s SCC machine. (c) A seller wants to sell an uninsured carbon credit (UICC). (d) A polluter wants to buy an insured carbon credit (ICC). (e) The RetroExchange picks the best counterparty to convert the UICC to ICC. This allows buyer and seller to execute the transaction. (f) During the transaction, the polluter pays for the carbon credit as well as the insurance policy. (g) RetroExchange and the counterparty exchange PReCaP adjustments over a future time period. (h) Counter-parties undergo SCC model innovation.
}
\label{fig:precap}
\end{figure}

We consider two types of sellers at the RetroExchange: (a) carbon credit supplier, and (b) the insurers who post the premium on these carbon credits.
First, there are sellers who have acquired the rights to sell carbon credits either by the way of a project that will, in the future, or has already captured a ton of carbon.
We call these uninsured carbon credits (UICCs).
The RetroExchange asks the insurance companies for a premium at which they could insure UICCs, following which the exchange selects the offer that provides the lowest premium. 
\textit{The optimal estimation of SCC is the lowest price that still allows the insurer to make money. 
Hence competitive bids combined with the need of the insurer to still make a profit will help favour those insurers who develop more accurate models.}
UICCs along with the insurer chosen by the RetroExchange, forms an insured carbon credits (ICCs).
Buyers bid on the RetroExchange for ICCs; UICCs are not directly purchasable. 
Finally, the selected insurer enters into a swap contract with the RetroExchange, thereby exchanging the ReSCCU adjustments on a periodic basis for a fixed period of time.

Insurers operate on the sell side of the exchange as they post the asked insurance premium and volumes of insurance contracts they are willing to sell. 
For simplicity, let's assume all retroactive payments are capped to $30$ years since conversion from UICC to ICC\footnote{Otherwise we need to distinguish between ICCs of different maturities}.
The clearing mechanism by the RetroExchange is now an auction with a complication: %sealed-bid 
While ICCs can be cleared straightforwardly, UICC clearance involves a form of transaction cost (or friction) due to the need to match bids and asks simultaneously with the lowest available policy insurance option. This transaction cost could be automatically applied by the exchange which would add the insurance costs to the spread. In principle, this form of "3-agent" transaction could be decomposed into two 2-agent transactions, where the buyer needs to present a previously acquired insurance certificate at the time of UICC acquisition. This, however, would allow polluters to strategically hedge insurance certificates, which may introduce a distorting effect on insurance policy pricing. A more detailed discussion of such an auction mechanism is beyond the scope of this paper.
%UICCs need to be cleared according to a novel 3-agent auction, i.e., the RetroExchange clearing mechanism needs to convert UICCs into ICCs according to whether the combined price of supplier ask and insurer premium asks can satisfy buyer bids. 

% The insurer premium can be regarded as a variable added transaction cost.
%Suppose we know the number of insurance contracts the insurers $j = 1\ldots J$ are willing to underwrite through the insurer specific supply function $S^j(p_t, \widehat{\text{SCC}}_{t_0}^{t_0})$, where $p$ is the premium. 
%Suppose we also know for each polluter $i=1,\ldots I$ the demand for credits as a function of the premium  and the initial SCC estimate.
%Generally, the premium $p_t$ is market-clearing when supply matches demand:

%\begin{equation}\label{equation:clearing}
%\begin{equation}
%\sum_j^{J} S^j(p_t, \widehat{\text{SCC}}_{t_0}^{t_0}) = \sum_i^{I} D^i(p_t, \widehat{\text{SCC}}_{t_0}^{t_0}).
%\end{equation}

%The choice of market mechanism determines how the market tries to find a market-clearing premium $p_t$. Many proposed mechanisms to find clearing prices are intractable unless the shape of demand and supply functions are constrained. 
%Without restricting the shape of demand and supply functions, organising an auction can be costly in terms of computation and communication between agents and the auction organisers. 
%In the real world, markets often operate mechanisms that are constantly in disequilibrium (such as the double auction), but which approximate the equilibrium prices nonetheless.
%Therefore, the choice of market mechanism, and the rationality with which the agents execute their orders in a disequilibrium market determine how successful the market is in satisfying agents preferences.

%In economic models, however, frequently convenient restrictions are placed on the supply- and demand-functions. 
%Oftentimes, demand is assumed to be decreasing in price. 

% Insurer competition is induced by the RetroExchange trying to minimise the combined asking price, i.e. insurer asks with lower premiums are preferred. 
% Winning insurance premium bids result in swap contracts (or new instruments NI) between the winning insurer and the RetroExchange. 






\subsection{Other incentives for participation}

A crucial aspect of PReCaP is that the participation in it is \textit{voluntary}, meaning that additional incentives are required in order for carbon credit buyers and sellers to be willing to pay for insurance surcharges. 
We argue that the following factors may plausibly incentivise voluntary participation in PReCaP:

\begin{itemize}
	\item \textbf{Corporate social responsibility (CSR):} It is conceivable that a number of large corporations would be willing to acquire a small share of their carbon credits through the RetroExchange for reasons of corporate social responsibility. This may incentivise polluters to expose at least a small share of their carbon credits to the PReCaP scheme.
	\item \textbf{Supplier support:} It is conceivable that a number of carbon credit suppliers may choose to exclusively sell through the RetroExchange for CSR (corporate social responsibility) or marketing reasons. As demand for carbon credits outstrips supply, this would then incentivise polluters to acquire any credits available even if subject to an insurance premium. 
    \item \textbf{Carbon credit pricing:} Institutional lenders, such as banks, require access to accurate long-term interest rate benchmarks. Such estimates would likely benefit from improved SCC forecasts. This may encourage banks to invest in PReCaP implementations.
	\item  \textbf{Risk Diversification}: In the literature on catastrophe risk it is shown that catastrophe risk insurance as an investment has small correlation to other market indices \footnote{Though it is unclear if this would hold for climate risks due to pollution as well, since there is a causal link between economic activity and carbon outputs.}. This may form financial incentives for insurance companies to participate in PReCaP schemes.
	\item \textbf{Regulatory incentives:} Governments, or supragovernmental organisations, could, in principle, introduce regulation incentivizing participation - for example by requiring all newly released voluntary carbon credits to be ReSCCU insured at first transaction - , or directly investing in, PReCaP implementations - this would require much less political buy-in than ReCaP, which, in addition would be much more easily scalable.
	\item \textbf{Charity and Philanthropy:} High net-worth individuals alone could subsidize small-scale PReCaP schemes. 
\end{itemize}

==> old/recap.tex <==
In this section, we discuss \textit{Retroactive Carbon Pricing (ReCaP)}, a concrete mechanism that seeks to implement ReSCCU in the context of carbon taxation with the help of participation from the government.
Our novel mechanism design incentivises the continuous innovation of retrospective climate damage estimates. 

At a basic level, ReCaP works as follows (see Figure \ref{fig:recap_basic}): First, the government enacts a retroactive carbon tax law that details the ReSCCU mechanism used to adjust the carbon tax over time. 
This mechanism may evolve with time but this will only affect future emissions.
The ReSCCU mechanism is devised by an independent modelling institution, which we name a \textit{RetroAgency}, and ratified by parliament.
After the carbon tax law comes into effect, polluters need to register their expected CO2 emissions for the ensuing year and pay the associated ReSCCU estimate according to the mechanism enshrined in law. 
Going forward indefinitely, after each additional year has passed, government and polluters exchange cash flows according to the ReSCCU adjustments.
This straightforward incorporation of ReSCCU into Pigouvian taxation does, in principle, expose polluters optimally to the best possible SCC estimation in the presence of epistemic uncertainty. 

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{images/recap_basic.png}
    \caption{Schematic depiction of idealized ReCaP. a) The government enacts a retroactive carbon tax law b) Polluters and government agree on next year's emissions volume c) Independent experts establish the best present SCC estimate d) Government taxes polluters according to the SCC estimate e) Polluters pollute while f) a year passes. g) Real-world climate damages from the past year are measured and adjustments to past year's SCC estimate are calculated h) Government and polluters settle SCC adjustments (also periodically over the coming years).}
    \label{fig:recap_basic}
\end{figure}

However, the above scheme has the following drawbacks : (a) How can individual polluters, in particular SMEs, manage the risks associated with ReSCCU adjustments?
Such companies do not have the skill, the expertise, the data nor the economies of scale to do predictive modeling of future climate damages caused by their current emissions, and (b) If the polluters go bankrupt sooner than the time period considered for ReSCCU, the polluters will not be paying the full cost of damages.
This can incentivise the participants to game the system. 
To safeguard against these shortcomings, we introduce the insurance companies in ReCaP to take over the risks (see Figure \ref{fig:recap})
% We therefore suggest a further modification to the basic ReCaP process: The introduction of insurance companies (see Figure \ref{fig:recap}). 

An insurance company uses its existing skills, resources, and economies of scale in order to establish a SCC prediction model to estimate the right premium for a policy product ahead of time, which, in equilibrium, should equal $\left(\text{SCC}_\infty-\text{SCC}_0\right)$ plus production costs. 
Importantly, ReCaP requires that several competing insurance companies undergo this process independently, creating a market for ReSCCU insurance policies available to polluters.
Polluters are now able to buy insurance against ReSCCU adjustments for their respective emissions on this market.
This makes polluters liable to a one-time insurance premium at the time of polution, after which they are no longer exposed to the risk of ReSCCU adjustments. 
Instead, \textit{the insurance companies settle any future cash flows with the government directly, overcoming the Tragedy of the Horizons by offloading risks to skilled market participants whose business models have always relied on long-term horizons.}

\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\linewidth]{images/ReCaP.png}
    \caption{The role of insurance companies in ReCaP. (a) An insurance company creates a SCC model to estimate the right premium for a policy product. (b) This happens at several insurance companies who compete on a market. (c) The polluter chooses the best available insurance policy product to insure its future pollution. (d) The insurance now takes over any ReSCCU adjustments between polluter and government. (e) A year passes. (f) Retrospective climate damages are measured, each insurance company may do this in a different way. (g) The insurance company innovates its models according to the new data. (h) The insurance company with the best SCC model can offer the lowest premiums.
}
    \label{fig:recap}
\end{figure}


\subsection{Opportunities}

Besides addressing the Tragedy of the Horizon issue, ReCaP also offers two additional attractive benefits - one fundamentally related to the Polluter Pays Principle, and the other addressing model innovation, a central challenge to SCC estimation.

\paragraph{Model innovation.} 
The need for ReSCCU is motivated by the fact that SCC is hard, or indeed impossible, to estimate accurately at the time of emission. 
While some of this difficulty arises from irreducible aleatoric environmental uncertainty, current SCC models almost certainly suffer from epistemic uncertainty, i.e.,  current models do not optimally process all relevant data that already is, or could be, available. 
The reason for this is clearly that there are insufficient incentives for model developers to create alternative integrated assessment models, or improve existing ones through either model innovation and/or additional data collection. 
While it is intrinsically unclear where exactly the boundary between aleatoric and epistemic modelling error lies, ReCaP can be seen to provide substantial financial incentives to insurance companies to continuously improve their ReSCCU forecasting models.

As insurance companies compete over polluter clients, in equilibrium, insurance premia offered will be equal to the marginal costs, which are likely dominated by ReSCCU $\Delta c_t$ adjustments. 
This means that insurance companies are incentivised to continuously innovate their models such as to reduce their forecasting error relative to future ReSCCU adjustments, which benefit from hindsight. 
Thus, insurance company surcharges arising in ReCaP can be interpreted as a precautionary investment in technological innovation, which, as other technological investments in e.g. renewable energy production, are justified even from a decentralised market perspective \citep{weisbach_should_2012}.

% What are large-scale ABM modeling techniques about? AI - EA Insights
% CIPR european network for economic analysis
% https://www.cbre.com/insights/ea-insights


\paragraph{Polluter-Pays Principle perspective.} Uncertainties surrounding greenhouse gas pollution also pose a number of questions when considering the implications of the \textit{polluter pays principle (PPP)} \citep{tokuc_rio_2013}, which is a statute of international environmental law that posits that 
\blockquote{\textit{National authorities should endeavour to promote the internalization of environmental costs and the
use of economic instruments, taking into account the approach that the polluter should, in principle,
bear the cost of pollution, with due regard to the public interest and without distorting international
trade and investment.}}
Isn't it unfair if polluters are charged according to estimated damages, rather than actual damages incurred? 
And should polluters be held responsible for sub-optimal future decision-making? 
For example, if a future government incentivises house building near the shore, naturally resultant property damages due to sea level rise may increase. 
As future decision-making could be arbitrarily ignorant, can we really make a polluter responsible for it at the time of emission? 
If not, what kind of future decision-making is the polluter liable to? By basing Pigouvian taxation rates on ReSCCU rather than SCC, many of these questions can be addressed optimally.


%In addition, we need additional incentives to collect all information that can be collected, and push model quality to the brink (i.e. it is unclear atm where the border is between aleatory and epistemic uncertainty in the context of SCC prediction so we need to invest lots of money into finding better models. I think we can interestingly here make the case that model development is endogenous to technological development, which would give another line of reasoning for why one should price it into taxes (as in Private ReCaP). Model innovation goes in here.
%\paragraph{Incentivising decision makers to behave predictably.} this is similar to "predictable flexibility" from finance. basically, multiagent theory tells us that even simple, well-define multiplayer games usually go chaotic, which means SCC is inherently unpredictable if that happens too much. I'd argue that ReCaP can incentivise decisionmakers to behave predictably as e.g. the discount rate is set low by Trump next year then that would create considerable backpayments for government, which I think would deter it from doing that. Likewise if government increases discount factor to make more money then insurance companies can bundle legal power to sue government effectively.




\subsection{Challenges}

While overcoming some issues of SCC-derived carbon taxes, ReCaP also poses a few practical challenges related to risk management as well as political buy-in and initial hurdles to implementation.

\paragraph{The limits of risk mitigation.} We have so far assumed that insurance companies can indeed estimate the total future ReSCCU adjustment, $\Delta c_t$, well enough in order to effectively price in risks through one-time premia at the time of CO2 emission. 
In fact, there are two main challenges in doing so: First, it is inherently unknown to what extent $\Delta c_t$ can be predicted, and whether it is indeed bounded. 
Second, insurance companies may find it difficult to diversify their climate risks as climate disasters tend to be correlated across regions and asset classes.
Various measures could be taken in order to offset risks to insurance companies.
Perhaps most straightforwardly, reinsurers, or, ultimately, governments, could choose to bear excess tail risks. 
This could be implemented by choosing a finite time horizon for $\Delta c_t$, introducing a  temporal discounting rate or simply through side contracts. 
While such measures would be successful in managing risk to insurers, they would at the same time dilute the efficacy of the Pigouvian taxation mechanism. 

\paragraph{Political buy-in and hurdles to practical implementation.} As a carbon taxation mechanism, ReCaP requires political buy-in from governments and insurance companies. 
Currently operating carbon taxation schemes tend to underprice CO2 emissions from a climate damage perspective, perhaps indicating limited political support for ReSCCU-like adjustments.

If the total insurance volume for ReCaP transactions becomes sufficiently large, the economic survival of insurance companies may started to be regarded as vital to financial and economic stability ("too big to fail"). 
This might dilute the perceived risks that insurance companies feel exposed to as they may bet on ultimately being bailed out by the government, potentially leading to artificially low premiums. 










% TODO: talk about convergence conditions etc (ReCaP in this context may not have any)
% Talk about insurance companies here!

%We now illustrate how ReCaP helps overcome a variety of challenges associated with current attempts to internalise marginal damages from GHG emission.

%TODO: The below paragraphs need to be reformulated.
%\paragraph{Dealing with environment uncertainty (aleatory uncertainty).} - in the context of PPP you should only pay for the damage that was actually created. also there's the question of precautionary principle wrt environment uncertainty and pigovian taxes.
%4:32
%\paragraph{Dealing with modeling uncertainty (epistemic uncertainty).} SCC is hard to calculate, models will change as our understanding improves. In addition, we need additional incentives to collect all information that can be collected, and push model quality to the brink (i.e. it is unclear atm where the border is between aleatory and epistemic uncertainty in the context of SCC prediction so we need to invest lots of money into finding better models. I think we can interestingly here make the case that model development is endogenous to technological development, which would give another line of reasoning for why one should price it into taxes (as in Private ReCaP). Model innovation goes in here.
%\paragraph{Incentivising decision makers to behave predictably.} this is similar to "predictable flexibility" from finance. basically, multiagent theory tells us that even simple, well-define multiplayer games usually go chaotic, which means SCC is inherently unpredictable if that happens too much. I'd argue that ReCaP can incentivise decisionmakers to behave predictably as e.g. the discount rate is set low by Trump next year then that would create considerable backpayments for government, which I think would deter it from doing that. Likewise if government increases discount factor to make more money then insurance companies can bundle legal power to sue government effectively.

%Taking all these complexities into account we, in this paper, argue that marginal climate damage estimation should be treated as a process endogenous to \textit{technological innovation and development}. 
%This suggests treating \textit{epistemic} innovation challenges similar in spirit to other technological innovation processes, such as renewable energy sources.

%Uncertainties surrounding greenhouse gas pollution also pose a number of questions when considering the implications of the \textit{polluter pays principle (PPP)} \citep{tokuc_rio_2013}, which is a statue of international environmental law that posits that 
%\blockquote{\textit{National authorities should endeavour to promote the internalization of environmental costs and the
%use of economic instruments, taking into account the approach that the polluter should, in principle,
%bear the cost of pollution, with due regard to the public interest and without distorting international
%trade and investment.}}
%Isn't it unfair if polluters are charged according to estimated damages, rather than actual damages incurred? 
%And in how far are polluters responsible for sub-optimal future decision-making? 
%For example, if a future government incentivises house building near the shore, naturally resultant property damages due to sea %level rise may increase. 
%As future decision-making could be arbitrarily ignorant, can we really make a polluter responsible for it at the time of emission? 
%If not, what kind of future decision-making is the polluter liable to?

==> old/resccu.tex <==
\label{sec:resccu}

\subsection{SCC is a moving target}
The marginal cost of future damages due to an extra ton of CO2 is difficult to estimate.
This is in part due to the fundamental aleatoric uncertainty in response of the physical world to future emissions and to the greater uncertainty on future decision making as well as socioeconomic pathways.
Since the marginal damage estimates form the basis for policy making there is a feedback loop tying today's estimate to tomorrow's created damage. 
For example, over-estimation of today's marginal damages may inflate the expectation of future damage estimates, thereby causing harsher policies to mitigate adverse effects resulting in lower than expected future damage.
The very existence of such feedback effects may already pose questions on whether a \textit{marginal damage} is indeed a well-definable concept, if not inherently tied to rigorous constraints on the nature of future decision making processes.

However, marginal damages are hard to estimate even when considering retrospective emissions.
Assuming a polluter emits an extra ton of CO2 at time $t$ and abates an extra ton of CO2 at future time $t'>t$, how exactly do we estimate the marginal damage caused even if the pollution event is assumed confined entirely to the interval $[t,t']$?
In order to understand this question better, we need to understand how climate damages occur. 

% mechanism of climate change and estimation of marginal damage - is tough
The mechanisms through which climate damage occurs are numerous. 
Among physical mechanisms, one may further distinguish between damages from extreme weather events, such as floods, hurricanes, and draughts, and events with more permanent effects, such as regional climate changes and sea level rise. 
Estimating damages from extreme weather events may seem comparably easy, given insurance and reinsurance companies do provide annual estimates of claims incurred. 
However, global insurance coverage is patchy and, particularly when considering livelihoods, does not cover many of the world's most vulnerable communities. 
In addition, not every extreme weather event is due to climate change. 
Even estimating last year's marginal damages from emitting an extra ton of CO2, the year before, is therefore difficult and relies on the emerging areas of climate attribution science \citep{otto_attribution_2016} and global quantitative estimates, such as those increasingly derived from automated earth observation \citep{jimenez-jimenez_rapid_2020}.

% attribution of damages from slow climate change events
Retrospective attribution of damages from sea level rise or regional climate change is equally difficult, and, apart from damages on physical assets, likewise requires inclusion of hard-to-quantify damage to human health (including psychological effects), biodiversity loss, and even quality of life. 
With data being unavailable, past attempts to quantify climate damage have largely relied on statistical methods comparing the economies of different climatic regions. 
Such approaches, however, inherently suffer from numerous confounding effects. 
A central problem concerns the costs incurred during adaptation.

% extrapolation of climate damages into the future
With climate damage hard to quantify retrospectively, extrapolating it into the future is naturally even harder. 
Firstly, the future transient climate response to rising levels of GHGs, while comparatively well-understood, inherently carries uncertainty. 
Secondly, future damages incurred depend on the particularities of future economies. 
We already noted how a future economy's adaptability and resilience to climate change influences the levels of damage incurred with respect to its physical effects, such as increases in the frequency of extreme weather events. 
Both these trends are compounded and inherently interlinked through the presence of countless decision makers in the system dynamics whose behaviour, even if their incentives and policies were fully known in advance, might readily drive system dynamics virtually unpredictable due to the emergence of bounded rationality effects \citep{botzen_bounded_2009}, system bifurcations such as those emerging from social tipping points \citep{otto_social_2020}, and, fundamentally, chaos arising naturally in multiplayer games \citep{sanders_prevalence_2018}. 
These fundamental constraints are largely ignored in current IAMs (see Section \ref{sec:iam}): For example, in DICE \citep{nordhaus_revisiting_2017}, population growth is treated as an exogenous variable - rather than an endogenous variable that should depend both on social dynamics as well as environmental constraints and effects \citep{stern_time_2021}.

% recap of why SCC estimation is tough
We have thus established that marginal damages from GHG emissions are intrinsically hard, or even impossible, to predict across sufficiently long time horizons given the numerous sources of \textit{aleatory}, i.e., environmental uncertainty. 
Even under optimistic assumptions, such as predictable decision making, exploiting any predictability poses hard \textit{epistemic}, i.e., modelling challenges: First, a lot of the required empirical data, even if theoretically measurable, is not currently available, and can often only be made available at significant cost. 
This issue ranges from a lack of weather and climate data in areas such as West Africa, up to insufficiently fine-grained economic data. 
Secondly, even if the necessary data was available, models would need to be run at sufficiently high resolution and scale, thus incurring complex model design and calibration challenges, as well as substantial computing costs. This emphasizes that significant financial incentives are required for model innovation.

\subsection{Formal Definition}

% Integrated assessment model development therefore needs to be endowed with the necessary resources, or otherwise economically incentivised. 
% Given the flaws of the current generations of IAMs, it is clear that, if \textit{model innovation} challenges are sufficiently addressed, marginal climate damage estimates will change over time, and, hopefully, monotonically improve - as long as current barriers to \textit{model adoption} are likewise resolved.
% In addition, quantifying marginal damages requires fundamental \textit{social value} choices that may directly influence the very utility objective to be optimised, for example DICE's infamous social discounting factor.
% Future climate damage estimates are thus tightly coupled to future political preferences and outcomes of democratic elections, where applicable.

In the wake of the above discussion, we introduce Restrospective SCC Updates (ReSCCU), to formalise the idea that SCC evaluations can, especially close to the time of emission, only ever be regarded as preliminary estimates.
It  posits that, after emitting a unit quantity of GHG emissions at time $t_0$, any initial SCC estimate, $\widehat{\text{SCC}}_{t_0}$, should be seen in anticipation of periodic future ReSCCUs, $\Delta_t$ at time $t$.
Thus, the true SCC, accounting for the present value of the sum total of future climate damages, is given by

\begin{equation}
    \text{SCC}_{t=t_0}^{t=\infty} = \widehat{\text{SCC}}_{t_0} + \sum\limits_{t=t_0+1}^{t=\infty}\underbrace{\widehat{\text{SCC}}_t - \widehat{\text{SCC}}_{t-1}}_{\Delta_t}
\end{equation}

Note that as the time since emission advances, our estimate of the true SCC becomes increasingly dominated by \textit{empirically measured} retrospective, rather than forecast, climate damages.

By requiring SCC estimates to always be considered jointly with future retroactive adjustments, ReSCCU, at first look, may seem to undermine the very utility of having SCC estimates, i.e., having access to a single number that can summarise a unit emission's future climate damages here and now. 
A more subtle consideration, however, reveals that ReSCCU reduces to the traditional notion of SCC precisely when the future damage estimation functions are exact, and deviates from the SCC estimates to the degree in which they are not. 
If we assume that our SCC estimation functions are largely correct, then we expect ReSCCU adjustments not to be significant.

While ReSCCU acknowledges the inherent uncertainty of SCC extending indefinitely into the future, it remains to be seen how this hypothetical and idealized concept can be implemented in the practical settings.
In the following sections, we propose two market-based mechanisms to implement PPP-conformant schemes through leveraging ReSCCU, while overcoming the inherent modelling inadequecies through \textit{model innovation}.


==> old/reverse_outline.tex <==
P1: (1) Climate change --> incentive misalignment

P2: (1a) Climate changes as `market failure' --> pricing GHG emissions to internalize damages

P3: (1b) Long-term decision-making --> Tragedy of the Horizons

P4: (1c) How to internalize (1a) and overcome TotH (1b) --> introduce argument that existing approaches fall short

P5: (2) Social cost of carbon --> Use in the US --> Limitations

P6: (2a) SCC limitations: (i) modeling limits + (ii) ethical, political choices on damage attribution and discounting

P7: (2b) Introduce carbon taxes --> set to SCC --> however, in practice, set to low rates + account for fraction of emissions

P8: (2c) Countries not using SCC --> difficult establishing around a single number --> Instead, target-consistent pricing more practical --> EU ETS as an example --> ETS limits: pricing inefficiencies

P9: (3) Voluntary carbon markets --> status of VCMs --> only subject to supply/demand, not realted to underlying GHG emissions damages

P10: (4) Many polluting economies subject to little-to-no carbon damage liabilities --> highlighting political barriers

P11: (5) Relevant long-term signal mechanisms in financial markets

P12: (5a) Interest rate benchmarks (LIBOR/SOFR) --> leveraged by long-term derivative --> need to follow Efficient Market Hypothesis, therefore, price climate damages

P13: (5b) Insurance markets --> lacks model innovation --> coverage varies and fragmented landscape --> thus, difficult to extract unbiased price signals

P14: (5c) Climate litigation --> emerging --> standardized market for litigation insurance

P15: (6) Summary --> existing approaches (i) do not couple prices to climate damages + (ii) suffer political risks and inherent modeling difficulties

P16: (7) Introduce ReCaP

1.2 Balancing Act: need to add intro paragraph on climate finance

1.3 CRA: (P1) Why we need better SCC, (P2) public sector use of SCC, (P3) Private sector use
